Joint Deep Learning for Improved Myocardial Scar Detection from Cardiac MRI

Automated identification of myocardial scar from late gadolinium enhancement cardiac magnetic resonance images (LGE-CMR) is limited by image noise and artifacts such as those related to motion and partial volume effect. This paper presents a novel joint deep learning (JDL) framework that improves such tasks by utilizing simultaneously learned myocardium segmentations to eliminate negative effects from non-region-of-interest areas. In contrast to previous approaches treating scar detection and myocardium segmentation as separate or parallel tasks, our proposed method introduces a message passing module where the information of myocardium segmentation is directly passed to guide scar detectors. This newly designed network will efficiently exploit joint information from the two related tasks and use all available sources of myocardium segmentation to benefit scar identification. We demonstrate the effectiveness of JDL on LGE-CMR images for automated left ventricular (LV) scar detection, with great potential to improve risk prediction in patients with both ischemic and non-ischemic heart disease and to improve response rates to cardiac resynchronization therapy (CRT) for heart failure patients. Experimental results show that our proposed approach outperforms multiple state-of-the-art methods, including commonly used two-step segmentation-classification networks, and multitask learning schemes where subtasks are indirectly interacted.

==> figures/intro-comparison.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/raw-images/intro/comparison.pdf}
    % \includesvg[width=\linewidth]{figures/raw-images/comparison.svg}
    % \includesvg{figures}
    \caption{Comparison of different approaches for scar segmentation}
    \label{fig:comparison}
\end{figure}

==> figures/method-pipeline.tex <==
\begin{figure}[h]
    \centering
    % \includegraphics[width=\linewidth]{figures/raw-images/pipeline.png}
    % \includesvg[width=\linewidth]{figures/raw-images/method/Pipeline2.svg}
    \includegraphics[width=\linewidth]{figures/Pipeline2.png}
    \caption{An overview of our proposed JDL framework}
    \label{fig:pipeline}
\end{figure}

==> figures/segmentation-Dice-table.tex <==
% Setting cell padding
% https://tex.stackexchange.com/questions/31672/column-and-row-padding-in-tables
\begin{table}[]
\centering
\def\arraystretch{1.1}
\setlength{\tabcolsep}{0.3em}
% \begin{tabular}{|c|cccc|}
% \hline
%           & Baseline & Multi-task & Two-step & Joint   \\ \hline
% Myocardium  & -        & 0.84264    & 0.82750  & \textbf{0.84306} \\
% Scar & 0.48918  & 0.48004    & 0.58200  & \textbf{0.66787}\\ \hline
% \end{tabular}
\begin{tabular}{|c|cccccccc|}
\hline
          & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{Two-step} & \multicolumn{2}{c}{Multi-task} & \multicolumn{2}{c|}{Joint}      \\ \hline
          & Mean         & Median        & Mean         & Median        & Mean          & Median         & Mean           & Median         \\ \hline
Myo Dice  & -            & -             & 0.828        & 0.855         & 0.828         & 0.827          & \textbf{0.843} & \textbf{0.869} \\
Scar Dice & 0.489        & 0.434         & 0.582        & 0.591         & 0.628         & 0.609          & \textbf{0.668} & \textbf{0.662} \\ \hline
\end{tabular} 
\caption{Segmentation Dice scores Statistics}
\label{table:mean-Dice}
\end{table}

==> refs-templet-bib <==
% @ARTICLE{Fortunato2010,
%   author  = {Fortunato, S.},
%   title   = {Community detection in graphs},
%   journal = {Phys. Rep.-Rev. Sec. Phys. Lett.}, 
%   volume  = {486},
%   year    = {2010},
%   pages   = {75-174}
% }

% @ARTICLE{NewmanGirvan2004,
%   author  = {Newman, M. E. J. and Girvan, M.},
%   title   = {Finding and evaluating community structure in networks},
%   journal = {Phys. Rev. E.}, 
%   volume  = {69},
%   year    = {2004},
%   pages   = {026113}
% }

% @ARTICLE{Vehlowetal2013,
%   author  = {Vehlow, C. and Reinhardt, T. and Weiskopf, D.},
%   title   = {Visualizing Fuzzy Overlapping Communities in Networks},
%   journal = {IEEE Trans. Vis. Comput. Graph.}, 
%   volume  = {19},
%   year    = {2013},
%   pages   = {2486-2495}
% }

% @ARTICLE{Raghavanetal2007,
%   author  = {Raghavan, U. and Albert, R. and Kumara, S.},
%   title   = {Near linear time algorithm to detect community structures in large-scale networks},
%   journal = {Phys. Rev E.}, 
%   volume  = {76},
%   year    = {2007},
%   pages   = {036106}
% }

% @ARTICLE{SubeljBajec2011a,
%   author  = {\v{S}ubelj, L. and Bajec, M.},
%   title   = {Robust network community detection using balanced propagation},
%   journal = {Eur. Phys. J. B.}, 
%   volume  = {81},
%   year    = {2011},
%   pages   = {353-362}
% }

% @ARTICLE{Louetal2013,
%   author  = {Lou, H. and Li, S. and Zhao, Y.},
%   title   = {Detecting community structure using label propagation with weighted coherent neighborhood propinquity},
%   journal = {Physica A.}, 
%   volume  = {392},
%   year    = {2013},
%   pages   = {3095-3105}
% }

% @ARTICLE{Clausetetal2004,
%   author  = {Clauset, A. and Newman, M. E. J. and Moore, C.},
%   title   = {Finding community structure in very large networks},
%   journal = {Phys. Rev. E.}, 
%   volume  = {70},
%   year    = {2004},
%   pages   = {066111}
% }

% @ARTICLE{Blondeletal2008,
%   author  = {Blondel, V. D. and Guillaume, J. L. and Lambiotte, R. and Lefebvre, E.},
%   title   = {Fast unfolding of communities in large networks},
%   journal = {J. Stat. Mech.-Theory Exp.}, 
%   volume  = {2008},
%   year    = {2008},
%   pages   = {P10008}
% }

% @ARTICLE{SobolevskyCampari2014,
%   author  = {Sobolevsky, S. and Campari, R.},
%   title   = {General optimization technique for high-quality community detection in complex networks},
%   journal = {Phys. Rev. E.}, 
%   volume  = {90},
%   year    = {2014},
%   pages   = {012811}
% }

% @ARTICLE{FortunatoBarthelemy2007,
%   author  = {Fortunato, S. and Barthelemy, M.},
%   title   = {Resolution limit in community detection},
%   journal = {Proc. Natl. Acad. Sci. U. S. A.}, 
%   volume  = {104},
%   year    = {2007},
%   pages   = {36-41}
% }

% @ARTICLE{SubeljBajec2011b,
%   author  = {\v{S}ubelj, L. and Bajec, M.},
%   title   = {Unfolding communities in large complex networks: Combining defensive and offensive label propagation for core extraction},
%   journal = {Phys. Rev. E.}, 
%   volume  = {83},
%   year    = {2011},
%   pages   = {036103}
% }

% @ARTICLE{WangLi2013,
%   author  = {Wang, X. and Li, J.},
%   title   = {Detecting communities by the core-vertex and intimate degree in complex networks},
%   journal = {Physica A.}, 
%   volume  = {392},
%   year    = {2013},
%   pages   = {2555-2563}
% }

% @ARTICLE{Lietal2013,
%   author  = {Li, J. and Wang, X. and Eustace, J.},
%   title   = {Detecting overlapping communities by seed community in weighted complex networks},
%   journal = {Physica A.}, 
%   volume  = {392},
%   year    = {2013},
%   pages   = {6125-6134}
% }

% @ARTICLE{Fabioetal2013,
%   author  = {Fabio, D. R. and Fabio, D. and Carlo, P.},
%   title   = {Profiling core-periphery network structure by random walkers},
%   journal = {Sci. Rep.}, 
%   volume  = {3},
%   year    = {2013},
%   pages   = {1467}
% }

% @ARTICLE{Chenetal2013,
%   author  = {Chen, Q. and Wu, T. T. and Fang, M.},
%   title   = {Detecting local community structure in complex networks based on local degree central nodes},
%   journal = {Physica A.}, 
%   volume  = {392},
%   year    = {2013},
%   pages   = {529-537}
% }

% @ARTICLE{Zhangetal2007,
%   author  = {Zhang, S. and Wang, R. and Zhang, X.},
%   title   = {Identification of overlapping community structure in complex networks using fuzzy c-means clustering},
%   journal = {Physica A.}, 
%   volume  = {374},
%   year    = {2007},
%   pages   = {483-490}
% }

% @ARTICLE{Nepuszetal2008,
%   author  = {Nepusz, T. and Petr\'oczi, A. and N\'egyessy, L. and Bazs\'o, F.},
%   title   = {Fuzzy communities and the concept of bridgeness in complex networks},
%   journal = {Phys. Rev. E.}, 
%   volume  = {77},
%   year    = {2008},
%   pages   = {016107}
% }

% @ARTICLE{FabricioLiang2013,
%   author  = {Fabricio, B. and Liang, Z.},
%   title   = {Fuzzy community structure detection by particle competition and cooperation},
%   journal = {Soft Comput.}, 
%   volume  = {17},
%   year    = {2013},
%   pages   = {659-673}
% }

% @ARTICLE{Sunetal2011,
%   author  = {Sun, P. and Gao, L. and Han, S.},
%   title   = {Identification of overlapping and non-overlapping community structure by fuzzy clustering in complex networks},
%   journal = {Inf. Sci.}, 
%   volume  = {181},
%   year    = {2011},
%   pages   = {1060-1071}
% }

% @ARTICLE{Wangetal2013,
%   author  = {Wang, W. and Liu, D. and Liu, X. and Pan, L.},
%   title   = {Fuzzy overlapping community detection based on local random walk and multidimensional scaling},
%   journal = {Physica A.}, 
%   volume  = {392},
%   year    = {2013},
%   pages   = {6578-6586}
% }

% @ARTICLE{Psorakisetal2011,
%   author  = {Psorakis, I. and Roberts, S. and Ebden, M. and Sheldon, B.},
%   title   = {Overlapping community detection using Bayesian non-negative matrix factorization},
%   journal = {Phys. Rev. E.}, 
%   volume  = {83},
%   year    = {2011},
%   pages   = {066114}
% }

% @CONFERENCE{ZhangYeung2012,
%   author  = {Zhang, Y. and Yeung, D.},
%   title   = {Overlapping Community Detection via Bounded Nonnegative Matrix Tri-Factorization},
%   booktitle = {In Proc. ACM SIGKDD Conf.}, 
%   year    = {2012},
%   pages   = {606-614}
% }

% @ARTICLE{Liu2010,
%   author  = {Liu, J.},
%   title   = {Fuzzy modularity and fuzzy community structure in networks},
%   journal = {Eur. Phys. J. B.}, 
%   volume  = {77},
%   year    = {2010},
%   pages   = {547-557}
% }

% @ARTICLE{Havensetal2013,
%   author  = {Havens, T. C. and Bezdek, J. C. and Leckie, C., Ramamohanarao, K. and Palaniswami, M.},
%   title   = {A Soft Modularity Function For Detecting Fuzzy Communities in Social Networks},
%   journal = {IEEE Trans. Fuzzy Syst.}, 
%   volume  = {21},
%   year    = {2013},
%   pages   = {1170-1175}
% }

% @misc{Newman2013,
%   author = {Newman, M. E. J.},
%   title  = {Network data},
%   howpublished = "\url{http://www-personal.umich.edu/~mejn/netdata/}",
%   year = {2013}
% }

% @ARTICLE{SubeljBajec2012,
%   author  = {\v{S}ubelj, L. and Bajec, M.},
%   title   = {Ubiquitousness of link-density and link-pattern communities in real-world networks},
%   journal = {Eur. Phys. J. B.}, 
%   volume  = {85},
%   year    = {2012},
%   pages   = {1-11}
% }

% @ARTICLE{Lancichinettietal2008,
%   author  = {Lancichinetti, A. and Fortunato, S. and Radicchi, F.},
%   title   = {Benchmark graphs for testing community detection algorithms},
%   journal = {Phys. Rev. E.}, 
%   volume  = {78},
%   year    = {2008},
%   pages   = {046110}
% }

% @ARTICLE{Liuetal2014,
%   author  = {Liu, W. and Pellegrini, M. and Wang, X.},
%   title   = {Detecting Communities Based on Network Topology},
%   journal = {Sci. Rep.}, 
%   volume  = {4},
%   year    = {2014},
%   pages   = {5739}
% }

% @ARTICLE{Danonetal2005,
%   author  = {Danon, L. and Diaz-Guilera, A. and Duch, J. and Arenas, A.},
%   title   = {Comparing community structure identification},
%   journal = {J. Stat. Mech.-Theory Exp.}, 
%   volume  = {},
%   year    = {2005},
%   pages   = {P09008}
% }

% @ARTICLE{Gregory2011,
%   author  = {Gregory, S.},
%   title   = {Fuzzy overlapping communities in networks},
%   journal = {J. Stat. Mech.-Theory Exp.}, 
%   volume  = {},
%   year    = {2011},
%   pages   = {P02017}
% }

% @ARTICLE{LancichinettiFortunato2009,
%   author  = {Lancichinetti, A. and Fortunato, S.},
%   title   = {Benchmarks for testing community detection algorithms on directed and weighted graphs with overlapping communities},
%   journal = {Phys. Rev. E.}, 
%   volume  = {80},
%   year    = {2009},
%   pages   = {016118}
% }

% @CONFERENCE{HullermeierRifqi2009,
%   author  = {Hullermeier, E. and Rifqi, M.},
%   title   = {A Fuzzy Variant of the Rand Index for Comparing Clustering Structures},
%   booktitle = {in Proc. IFSA/EUSFLAT Conf.}, 
%   year    = {2009},
%   pages   = {1294-1298}
% }


==> sections/00.Template.tex <==
\section{Note}
\label{sec1}
Please use \verb+elsarticle.cls+ for typesetting your paper.
Additionally load the package \verb+medima.sty+ in the preamble using
the following command: 
\begin{verbatim} 
  \usepackage{medima}
\end{verbatim}

Following commands are defined for this journal which are not in
\verb+elsarticle.cls+. 
\begin{verbatim}
  \received{}
  \finalform{}
  \accepted{}
  \availableonline{}
  \communicated{}
\end{verbatim}

Any instructions relavant to the \verb+elsarticle.cls+ are applicable
here as well. See the online instruction available on:
\makeatletter
\if@twocolumn
\begin{verbatim}
 http://support.stmdocs.com/wiki/
 index.php?title=Elsarticle.cls
\end{verbatim}
\else
\begin{verbatim}
 http://support.stmdocs.com/wiki/index.php?title=Elsarticle.cls
\end{verbatim}
\fi

\subsection{Entering text}
\textcolor{newcolor}{\bf There is no page limit.}

\section{The first page}
Avoid using abbreviations in the title. Next, list all authors with
their first names or initials and surnames (in that order). Indicate
the author for correspondence (see elsarticle documentation).

Present addresses can be inserted as footnotes. After having listed all
authors' names, you should list their respective affiliations. Link
authors and affiliations using superscript lower case letters.

\subsection{The Abstract}
An Abstract is required for every paper; it should succinctly summarize
the reason for the work, the main findings, and the conclusions of the
study. The abstract should be no longer than 200 words. Do not include
artwork, tables, elaborate equations or references to other parts of
the paper or to the reference listing at the end. ``Comment'' papers
are exceptions, where the commented paper should be referenced in full
in the Abstract.

The reason is that the Abstract should be understandable in itself to
be suitable for storage in textual information retrieval systems.

\textit{Example of an abstract: A biometric sample collected in an
uncontrolled outdoor environment varies significantly from its
indoor version. Sample variations due to outdoor environmental
conditions degrade the performance of biometric systems that
otherwise perform well with indoor samples. In this study, we
quantitatively evaluate such performance degradation in the case
of a face and a voice biometric system. We also investigate how
elementary combination schemes involving min-max or z
normalization followed by the sum or max fusion rule can
improve performance of the multi-biometric system. We use
commercial biometric systems to collect face and voice samples
from the same subjects in an environment that closely mimics the
operational scenario. This realistic evaluation on a dataset of
116 subjects shows that the system performance degrades in
outdoor scenarios but by multimodal score fusion the
performance is enhanced by 20\%. We also find that max rule
fusion performs better than sum rule fusion on this dataset. More
interestingly, we see that by using multiple samples of the same
biometric modality, the performance of a unimodal system can
approach that of a multimodal system.}

\section{The main text}

Please divide your article into (numbered) sections (You can find the
information about the sections at
\url{http://www.elsevier.com/wps/find/journaldescription.cws_home/505619/authorinstructions}).
Ensure that all tables, figures and schemes are cited in the text in
numerical order. Trade names should have an initial capital letter, and
trademark protection should be acknowledged in the standard fashion,
using the superscripted characters for trademarks and registered
trademarks respectively. All measurements and data should be given in
SI units where possible, or other internationally accepted units.
Abbreviations should be used consistently throughout the text, and all
nonstandard abbreviations should be defined on first usage
\citep{Vehlowetal2013}.

\begin{table*}[!t]
\caption{\label{tab1}Summary of different works pertaining to face and
speech fusion}
\centering
\begin{tabular}{|p{2.25cm}|p{2cm}|l|p{4cm}|p{3cm}|p{2cm}|}
\hline
Study & Algorithm used & DB Size & Covariates of interest & 
Top individual performance & Fusion\newline Performance\\
\hline
UK-BWG
(Mansfield et al.,
2001) &
Face, voice:\newline
Commercial & 200 & Time: 1--2 month\newline
separation (indoor) & 
TAR$^*$ at 1\% FAR$^{\#}$\newline
Face: 96.5\%\newline
Voice: 96\%
& --\\
\hline
Brunelli
(Brunelli and
Falavigna, 1995) & 
Face:\newline
Hierarchical\newline
correlation\newline
Voice:\newline
MFCC & 
87 & 
Time: 3 sessions, time\newline
unknown (indoor) & 
Face:\newline
TAR = 92\% at\newline
4.5\% FAR\newline
Voice:\newline
TAR = 63\% at\newline
15\% FAR
&
TAR =98.5\%\newline
at 0.5\% FAR\\
\hline
Jain
(Jain et al., 1999)
&
Face:\newline
Eigenface\newline
Voice:\newline
Cepstrum\newline
Coeff. Based
&
50
&
Time: Two weeks (indoor)
&
TAR at 1\% FAR\newline
Face: 43\%\newline
Voice: 96.5\%\newline
Fingerprint: 96\%
& 
Face $+$ Voice $+$\newline
Fingerprint $=$\newline
98.5\%\\
\hline
Sanderson
(Sanderson and
Paliwal, 2002)
&
Face: PCA\newline
Voice: MFCC &
43 
& Time: 3 sessions (indoor)\newline
Noise addition to voice & 
Equal Error Rate\newline
Face: 10\%\newline
Voice: 12.41\%
&
Equal Error\newline
Rate 2.86\% \\
\hline
Proposed study & 
Face, voice:\newline
Commercial & 116 &
Location: Indoor and\newline
Outdoor (same day)\newline
Noise addition to eye\newline 
coordinates 
&
TARs at 1\% FAR\newline
Indoor-Outdoor\newline
Face: 80\%\newline
Voice: 67.5\%
&
TAR = 98\%\newline
at 1\% FAR\\
\hline
\multicolumn{6}{@{}l}{$^*$TAR--True Acceptance Rate\qquad 
$^{\#}$ FAR--False Acceptance Rate}
\end{tabular}
\end{table*}


\subsection{Tables, figures and schemes}
Graphics and tables may be positioned as they should appear in the
final manuscript. Figures, Schemes, and Tables should be numbered.
Structures in schemes should also be numbered consecutively, for ease
of discussion and reference in the text. \textcolor{newcolor}{\bf
Figures should be maximum half a page size.}

Depending on the
amount of detail, you can choose to display artwork in one column (20
pica wide) or across the page (42 pica wide). Scale your artwork in
your graphics program before incorporating it in your text. If the
artwork turns out to be too large or too small, resize it again in your
graphics program and re-import it. The text should not run along the
sides of any figure. This is an example for citation \citet{NewmanGirvan2004}.

\begin{figure}[!t]
\centering
\includegraphics[scale=.5]{medimafig01}
\caption{Studio setup for capturing face images indoor. Three light
sources L1, L2, L3 were used in conjunction with normal office lights.}
\end{figure}

You might find positioning your artwork within the text difficult
anyway. In that case you may choose to place all artwork at the end of
the text and insert a marker in the text at the desired place. In any
case, please keep in mind that the placement of artwork may vary
somewhat in relation to the page lay-out \citep{HullermeierRifqi2009}.

This can easily be achieved using \verb+endfloat.sty+ package. Please
refer the following documentation to use this package.
\makeatletter
\if@twocolumn
\begin{verbatim}
  http://mirrors.ctan.org/macros/latex/contrib/
  endfloat/endfloat.pdf
\end{verbatim}
\else
\begin{verbatim}
  http://mirrors.ctan.org/macros/latex/contrib/endfloat/endfloat.pdf
\end{verbatim}
\fi
\makeatother

\textcolor{newcolor}{\bf You should insert a caption for the figures
below the figures and for the tables the caption should be above the
tables.} 

Please remember that we will always also need highresolution versions
of your artwork for printing, submitted as separate files in standard
format (i.e. TIFF or EPS), not included in the text document. Before
preparing your artwork, please take a look at our Web page:
\url{http://www.elsevier.com/locate/authorartwork}.


\subsection{Lists}

For tabular summations that do not deserve to be presented as
a table, lists are often used. Lists may be either numbered or
bulleted. Below you see examples of both.
\begin{enumerate}
\item The first entry in this list
\item The second entry
\begin{enumerate}
\item A subentry
\end{enumerate}
\item The last entry
\end{enumerate}
\begin{itemize}
\item A bulleted list item
\item Another one
\end{itemize}

\subsection{Equations}
Conventionally, in mathematical equations, variables and
anything that represents a value appear in italics.
All equations should be numbered for easy referencing. The number
should appear at the right margin.
\begin{equation}
S_{\rm pg}'=\frac{S_{\rm pg}-\min(S_{\rm pG})}
 {\max(S_{\rm pG}-\min(S_{\rm pG})}
\end{equation}
In mathematical expressions in running text ``/'' should be used for
division (not a horizontal line). 

\section*{Acknowledgments}
Acknowledgments should be inserted at the end of the paper, before the
references, not as a footnote to the title. Use the unnumbered
Acknowledgements Head style for the Acknowledgments heading.

\section*{References}

Please ensure that every reference cited in the text is also present in
the reference list (and vice versa).

\section*{\itshape Reference style}

Text: All citations in the text should refer to:
\begin{enumerate}
\item Single author: the author's name (without initials, unless there
is ambiguity) and the year of publication;
\item Two authors: both authors' names and the year of publication;
\item Three or more authors: first author's name followed by `et al.'
and the year of publication.
\end{enumerate}
Citations may be made directly (or parenthetically). Groups of
references should be listed first alphabetically, then chronologically.

%%Harvard
\bibliographystyle{model2-names.bst}\biboptions{authoryear}
\bibliography{refs}

\section*{Supplementary Material}

Supplementary material that may be helpful in the review process should
be prepared and provided as a separate electronic file. That file can
then be transformed into PDF format and submitted along with the
manuscript and graphic files to the appropriate editorial office.
